Securing Parallel-chain Protocols under Variable Mining Power

Several emerging PoW blockchain protocols rely on a "parallel-chain" architecture for scaling, where instead of a single chain, multiple chains are run in parallel and aggregated. A key requirement of practical PoW blockchains is to adapt to mining power variations over time. In this paper, we consider the design of provably secure parallel-chain protocols which can adapt to such mining power variations. The Bitcoin difficulty adjustment rule adjusts the difficulty target of block mining periodically to get a constant mean inter-block time. While superficially simple, the rule has proved itself to be sophisticated and successfully secure, both in practice and in theory. We show that natural adaptations of the Bitcoin adjustment rule to the parallel-chain case open the door to subtle, but catastrophic safety and liveness breaches. We uncover a meta-design principle that allow us to design variable mining difficulty protocols for three popular PoW blockchain proposals (Prism, OHIE, and Fruitchains) inside a common rubric. The principle has three components:(M1) a pivot chain, based on which blocks in all chains choose difficulty, (M2) a monotonicity condition for referencing pivot chain blocks and (M3) translating additional protocol aspects from using levels (depth) to using "difficulty levels". We show that protocols employing a subset of these principles may have catastrophic failures. The security of the designs is also proved using a common rubric - the key technical challenge involves analyzing the interaction between the pivot chain and the other chains, as well as bounding the sudden changes in difficulty target experienced in non-pivot chains. We empirically investigate the responsivity of the new mining difficulty rule via simulations based on historical Bitcoin data, and find that the protocol very effectively controls the forking rate across all the chains.

==> prelim.tex <==
\section{Preliminary}

We call the threshold of the hash inequality in proof-of-work mining the {\it target} of a block. For a chain $\C$ formed of blocks $B_1, B_2, \cdots, B_n$ with targets $T_1, T_2, \cdots, T_n$, let the accumulated difficulty of chain $\C$ be ${\rm diff}(\C) = \sum_{i=1}^n 1/T_i$. Then we can see each block covers an interval of difficulty. For example, block $B_j$ in chain $\C$ covers interval $(\sum_{i=1}^{j-1} 1/T_i, \sum_{i=1}^j 1/T_i]$.

==> revisions.tex <==
{\color{red}
\noindent Major revisions:
\begin{itemize}
    \item As suggested by the reviewers, we have reorganized the proof structure in a unified manner. The proofs are divided into three parts: (a) pivot chain properties, (b) non-pivot chain properties, (c) full protocol security. All three protocols need (a), \scheme and {
    \sf OHIE} need (b), and (c) depends on the specific ledger formation rule in each protocol.
    \item We have revised and motivated the definitions systematically; we added a table of  important notations (Table \ref{tbl:notation}).
    \item We added a proof sketch sooner (Section \ref{sec:sketch}) without complicated notations and definitions.
    \item We have justified the selections of parameters for all three protocols.
    \item We explained a simple attack in Appendix \ref{app:attack} as a prelude to the difficulty raising attack. This should help understanding the attacks on \scheme in Section \ref{sec:prism}. 
    \item We performed a detailed analysis of the computational and storage overhead of our scheme. The analysis is backed by empirical data from a full stack  implementation of \scheme in \cite{prism-system} and a new simulation experiment.
    \item We clarified the experimental setup and metrics, and reorganized Section \ref{sec:exp-setup} to better present it.
\end{itemize}

\noindent Minor revisions:
\begin{itemize}
    \item In Figures \ref{fig:ohie_fixed} and \ref{fig:ohie_variable}, we specified the order in which blocks arrive for completeness.
    \item We give an example of the ledger formation rule of Prism in Figure \ref{fig:prism_ledger}.
    \item For all figures, we have ensured completeness of labels and captions for clearer comprehension.  
\end{itemize}

\noindent Other comments:
\begin{itemize}
    \item A crucial piece of notation caused  confusion during the review process. We have now highlighted this notation upfront in  Section \ref{sec:intro}  and tabulated it for extra emphasis. We repeat it for completeness:  The {\em block difficulty} of a block is measured in terms of how many times the block is harder to obtain than using the initial target of the system that is embedded in the genesis block. The {\em chain difficulty} of a chain is the sum of block difficulties of all blocks that comprise the chain. The chain difficulty of a block is the chain difficulty of the chain ending at this block.
\end{itemize}
}
\subsection*{Final comments}

The reviewers overall think the paper would make a fine contribution for CCS. However, there are a number of aspects that need to be addressed in a revision. Please make sure to address them thoroughly before resubmitting.

\noindent{\bf Definitions} Please revise all the definition used. Clarify your general principles, in particular M2, and their motivation. For M2, explain how the increasing difficulty deals with scenarios when the popularity of the system and hence the combined computational power decreases. \re{We revised and motivated the definitions, and also the general principles. For M2, increasing (or non-decreasing) difficulty refers to chain difficulty (i.e., the sum of block difficulties in a chain). So even when the combined computational power decreases, the chain difficulty of the pivot chain will still increase as the chain grows. This is now made very clear.}

\noindent {\bf Proofs} There were a number of issues raised with your proofs, please revise the proofs to address them. Here are the more major comments, please also include smaller comments from the reviews and requests for clarification from the reviews:

1) Explain the selection of the parameters $\Phi$, l, and s in equation 2-4 (on page 9) for Prism, the parameters in equation 8 (on page 17) for Fruitchains. Are those parameters the best lower bounds or upper bounds? \re{We have  justified the selections of parameters in Section \ref{sec:def} and Appendix \ref{app:fruit}. These parameters are not necessarily the best (upper or lower) but they  are sufficient for the security of the variable difficulty mining rule, as shown mathematically in this paper. Tightening these parameters for efficiency is outside the scope of this paper.}

2) What are the parameters $\Phi$, l and s corresponding to Eq. 2-4 for OHIE if something comparable exists? \re{The parameters for \ohie is the same as \schemenosp. This is now made clear.}

3) As you claim fairness for OHIE, please include a proof of it (or make it clearer if you think it is already in the current version). \re{We do not claim fairness for \ohie  (there was a typo in early submission). We only claim fairness for \fruitchains (the proof is in Appendix \ref{app:fruit}).}

4) Clarify the adversarial model with regard to (fraction of) honest, rational, and Byzantine nodes. \re{In our  model there are only two types of nodes: honest and Byzantine. Incentive and rational behavior are the outside the scope of this paper. The security of the variable difficulty mining rule is proved under the condition that the  Byzantine nodes have less mining power than honest nodes {\em at all time}, i.e., ``honest majority''. This is clarified in Section \ref{sec:model}.}

We also recommend summarizing the proving properties, the proof sketch, and the chosen parameters of each protocol in, e.g., a table, before going into the details of the individual proofs. \re{We added a proof sketch early on (in Section \ref{sec:sketch})  without complicated notations and definitions. The parameters used in our analysis are now  tabulated (in Table \ref{tbl:notation}).}

\noindent {\bf Evaluation of Overhead} Please provide empirical evidence of the claim that your scheme does not add considerable overhead and explore how the overhead depends on the parameters. \re{We added a detailed analysis of computation and storage overhead in Section \ref{sec:overhead}. We use empirical results from \cite{prism-system} to justify  our claim regarding storage overhead, and perform a new simulation to justify  the claim on computational overhead.}

\noindent {\bf Clarity of Evaluation} Please describe the general protocol used in the evaluation in sufficient detail, clarify the metrics and settings (e.g., latency) used. Ensure all the figures are readable. \re{We reorganized Section \ref{sec:exp-setup} to provide comprehensive details on the simulation testbed, which has enhanced  readability.}

\subsection*{Reviewer A}

\noindent {\bf Weaknesses}
\begin{itemize}
    \item Some of the definitions are a bit vague. Many definitions with little motivation \re{We have revised and motivated the definitions systematically; this includes the definitions of {\em block difficulty} and {\em chain difficulty}.} 
    \item Unsure where proofs include adversarial behaviour. \re{Our security proof is against all attacks on the consensus layer: the adversary can mine any content in the block, release blocks at their chosen time, fake timestamp. Furthermore, the adversary can also delay messages within a bound. In the proof, we show that safety/liveness failure occur with negligible probability as long as the adversary controls less than a majority of mining power. This is clarified in Section \ref{sec:model}.}
    \item Simulation setting not full described. \re{We have reorganized Section \ref{sec:exp-setup} to provide comprehensive details on the simulation testbed, which has enhanced  readability.}
\end{itemize}


\noindent {\bf Comments for author}
The paper identifies a design issue common to many parallel-chain protocols. It then performs an analysis all these protocols can benefit from, so it's both a neat observation and is applicable for a range of protocols.

All my issues essentially erase from the same issue: I found the paper very hard to follow. The language is mostly fine but the amount of detail and the structure is sometimes difficult.

One obvious issue here is that not knowing all the different protocols in detail makes it harder to understand the modifications. That seems hard to avoid and I found that part of the paper still reasonably clear, so I am going to focus on the other aspects.

First, the definitions of M1-M3 are not very precise. In particular, I initially understood M2 as stating that the difficulty has to always increase, which did not make sense. After reading the paper, I now think it means that the number of the pivot chain referred to has to increase, but I am not entirely certain, which is a pity given the importance of the property. \re{Chain-difficulty is the total difficulty of the chain (i.e., the summation of block difficulties in the chain). M2 requires that the chain-difficulty of the referred pivot chain has to be non-decreasing in any non-pivot chain. We now clearly separate block difficulty from chain difficulty in Section \ref{sec:intro}; thank you for raising this important point, without which the contributions of the paper are indeed very hard to follow.}

Second, I struggled with the security analysis and did at times get too lost to trust that I verified the claims. First, the section starts with many definitions and a lot of variables without giving much of an indication on the intuition and purpose of them. \re{We have added a proof sketch earlier in Section \ref{sec:sketch} without complicated notations and definitions.} I was pretty lost about where it was going, though Figure 8 helped. Sadly, I encountered it pretty late and adding lemma/theorem numbers for each of the results would have helped to map it to the text. In Section 6.3, there were a lot of statements about the variables, which I fail to understand why they should hold, particularly Eq. 2. A lot of the proofs seem to be focused on honest nodes as well, I am unsure to what extent malicious behaviour is considered. \re{The adversarial model is the standard  Byzantine model, where there are two types of nodes: honest (follow protocol) and Byzantine (can deviate from protocol in any manner). We require that the  fraction of honest mining power be greater than 50\% at all times; this  is clarified in Section \ref{sec:model}.} Sometimes the phrasing here is vague/insufficiently defined, e.g., what does it mean if a chain is held by honest parties? \re{A chain is called ``held by honest parties'' if it is held by at least one honest party as the heaviest chain. We clarified this  in Notation ~\ref{notation:chains}; we  also clarify that the analysis goes beyond just the chains held by honest parties in Section ~\ref{sec:def}} Are all parties honest or the majority? \re{Similar to Bitcoin, the security of all three protocols necessarily requires the honest majority assumption. This is clarified in Section \ref{sec:model}.} While it is probably not possible to avoid the notation, a notation table and more motivation would have helped. \re{The parameters used in our analysis are now listed in Table \ref{tbl:notation}.} I kept searching for terms whose meaning I forgot.

Third, I don't fully understand the simulation study, at least not to the extent that I can reproduce it. It says that it's using the new `scheme' in a general setting, not specific to any of the protocols before. However, there was no generic scheme introduced before, only how to integrate the three principles into OHIE, Prism, and Fruitchains. So, I am unsure how exactly that simulated scheme works. Furthermore, the paper states that it uses data from Bitcoin and Prism but it's not clear to me which data is from Prism and whether the historical data on mining difficulty is the only data from Bitcoin or if there is more. There is also the sentence `In each round, blocks are mined on each of the parallel chains by drawing from Poisson random variable.' Is that one Poisson random variable per user, per chain, globally? If any of the last two, how do you choose the users? \re{We simulate the mining process of parallel chains, which is common to all parallel-chain protocols and hence being general. In this revision, we made this point more clear and included more detail on the simulated protocol in Section \ref{sec:exp-setup}. We use network latency data from Prism, and use historical mining power data from Bitcoin. This is clarified in this revision. We simulate two parties, honest and adversary and the randomness involved in their mining activity}. 

Fourth and more minor, the evaluation states it considers `heavy attack'. The attack described is pretty simple, is that the best attackers can do? \re{While private attacks are  the best attacks on the longest chain protocol in some conditions, it is not clear what  the best attacks are in PCPs. We have simulated the natural analog of the private attacks on PCPs (whose efficacy is measured via the  forking rate), while varying the adversarial mining power. %\xw{Is this true? I think we did not simulate private attack.}
}

Nitpicks: \re{All addressed. Thank you for catching them and mentioning them to us.}

The paper writes sets of integers as intervals, which for me is a common notation for real numbers.

Sometimes subsets are denoted as elements, e.g., $S \in [0,r]$ rather than $S \subset [0,r]$ (Def. 2.1). 

Spaces between max/min and the variables after would improve readability (e.g., Def. 2.1).

Figure 1: what do the different colours for the 'reference link to vote' mean? \re{No special meaning. We now use only one color.}

Definition 6.2: `then it holds that honest blocks in $C(S_0)$ have total difficult at least $\mu d$.' -> total difficulty? Maybe cut the definition in two sentence, it's a hard-to-read 6-line sentence.

Definition 6.3: with timestamp in last -> in the last.

P.9: compared to duration -> compared to the duration.

Questions for authors’ response
How exactly does the simulated protocol work? \re{We simulate the mining process of parallel chains, as a general skeleton common to all parallel-chain protocols. Two parties, honest and adversary, mine blocks on all parallel chains at the same mining rate, and we enforce the rules \textbf{M1}, \textbf{M2}. In this revision, we made this point  clearer and included more detail on the simulated protocol in Section \ref{sec:exp-setup}. We do not simulate transaction confirmation.}

\subsection*{Review B}
\noindent {\bf Weaknesses}
\begin{itemize}
    \item One challenge in reading the paper is that it aims to cover so much content (within page limit) that some important technical details are underspecified or relegated to appendices. That hampers understanding in my opinion and is my main sources of complains. \re{It is true that substantial technical material has been developed in the paper for the novel fork choice rule and corresponding security analysis. In this revision, we have consolidated the proof methods, providing a common methodology across all 3 types of parallel chain protocols. We also provide a sketch of the proof and a consolidated table of notations. We expect these revisions to address this important point. }
    \item The proof is very hard to follow without reading [11,13, 3] first. The lack of clarity (previous point) makes it worse. \re{We reorganized the proof quiet a bit, also motivated and clarified definitions. Much of the proof is common to all three  protocols, and  only the last step of the proof requires the details of each of the three specific protocols. These changes should make the proof more readable.}
    \item The experiment seems a bit arbitrary. It's unclear why those evaluations are chosen and how they relate to the properties that we care about in practice. Moreover, despite the claim that ``our variable difficulty scheme does not add significant computation and communication overhead,'' authors do not provide empirical evidence. \re{We point out the best attack on a variable-difficulty parallel-chain is an open problem, so we do not try to evaluate the best attack. On the other hand, the metrics reported (forking rate) represents the vulnerability to the private mining attack, which indeed has been shown to be the worst case attack on the basic longest chain protocol in certain network regimes. Regarding the overhead, we have added a new Section \ref{sec:overhead} with detailed analysis backed by experimental results reported by \cite{prism-system} and new simulations. }
\end{itemize}


\noindent {\bf Comments for author}
Section 3: I think the difficulty raising attack and anti-centralization argument in Appendix 1 are important, because they are prerequisites (for me at least) to understanding arguments around M2 and the attack in Fig 2. Since they are needed for multiple basic things, they should perhaps appear in the main body. \re{Thank you for the suggestion. We tried our best but space limitations prevented us from moving the description of this attack to the main body.}

After consulting the appendix, I still can't reconcile the attacks M2 is meant to prevent and the difficulty raising attack in Fig 2. The first confusing thing is the conflicting description about the attack: Fig 2 refers to the proposer-parent as ``from the past'', but the text in the left column says ``at the current time [...] the adv will refer to this very difficult block''. Which way is it: a proposer-parent from the past or the current time? \re{At the current time on the non-pivot chain, the adversary will refer to a block on the pivot chain whose timestamp is in the past and has a high block-difficulty. We updated the figure description to address this.} Secondly, the goal of M2 is to force miners to use the latest difficulty, but why does that necessarily prevent the attack in Fig 2? Note that an adversarial proposer block is not necessarily a stale one, i.e., it could be the block with non-decreasing chain difficulty if it's recently mined, no? Please elaborate why M2 prevents the attacks and how it is reflected in the security proof. \re{At a high level, to launch this attack, the adversary needs to refer to an extremely difficult proposer block. With M2, the adversary can only refer to a non-stale one, which always has reasonable difficulty (close to difficulty of the block at the tip) by the security of Bitcoin rule;  hence the attack is prevented. This logic  can now be found in Section \ref{sec:strawman} and in the proof sketch (Section \ref{sec:sketch}); thank you for suggesting this idea.}

The ledger formation rule is also underspecified. First of all its unclear how to ``sanitize them into disjoint intervals''. So is the definition of g(.) as it involves several underspecified steps. Please elaborate. An example would help tremendously. \re{Thank you for the suggestion. We have added Figure \ref{fig:prism_ledger} to explain the sanitization step.}

Section 4: Fig 5: you need to specify the order in which blocks arrive for completeness. \re{Thanks for the suggestion. Addressed.}
Section 6: I found the proof very difficult to read, partly because it heavily involves the specifics of [3,11,13] (Like what is $head(C\cup C')$? I couldn't even find a definition \re{The definition of $head(C\cup C')$ can be found in Section \ref{sec:prop} now. Thanks for pointing out this.}), but also because the clarify issues in Section 3. I'm able to get a gist of what's going on from Figure 8, but frankly the rest of the Section 6 is not really readable. One suggestion is to consider moving section 6.4 upfront, so readers know what's about to happen. \re{Thanks for the suggestion. We took this wholeheartedly: we  added a proof sketch early on (in Section \ref{sec:sketch}) without complicated notations and definitions and consolidated the proof for all three protocols under one common rubric.} Moreover, since the methodology is generic for many blockchains, I wonder if it is possible to simplify the proof by exploiting the common structure of these protocols, i.e., to prove security w.r.t. to a more abstract model that captures the essence of all three without going to ``low levels'' like [11,13]? \re{Thanks for the suggestion; we reorganized the proof structure in a unified manner. The proofs are divided into three parts: (a) pivot chain properties, (b) non-pivot chain properties, (c) full protocol security. All three protocols need (a), Prism and OHIE need (b), and (c) depends on the specific ledger formation rule in each protocol.}

Section 7: The big question is why you chose to simulate these attacks, which are much less sophisticated than, e.g., fig 2. \re{Please see the response below.} Interestingly, however, I found these experiments gives me a better understanding of the design goal than Section 3.1 did. I suggest you mention these (simpler) attacks upfront in Section 3. \re{Thanks for the suggestion. We added reference to the simulation results at the end of Section 3.2.} A few more comments below.
\begin{itemize}
    \item Isn't figure 14 mostly benchmarking the the difficulty adjustment rule of [13]? Without adversary it's expected that voter chains copy the difficulty rather promptly, no? Would be interesting to see the same graph with adversary. \re{The idea of Fig. 14 is to show that voter chains update their mining difficulty quickly, following updates on proposer chains. The green curve is a region that covers the difficulty of all voter chains at a given time. To answer your question regarding behavior under adversary presence, please see Fig. 12. It plots the time between pivot chain updating difficulty and non-pivot chain updating.}
    \item Fig 13 shows only the frequency but that's only one aspects of the story. At least I wonder about magnitude. But I'm not sure if frequency or magnitude is a good indicator. At the end of the day we care about attacker's advantage, which is not reflected here. \re{The magnitude is high in this attack. This is because the attacker’s block would adopt the difficulty of whatever pivot-chain block it is mined on, so the attacker can choose any difficulty that has appeared since the genesis block. So we decided to focus on the frequency. The point that we do not show the real advantage of the attacker is well-taken; however, the   best strategy for an attacker to utilize such difficulty fluctuation is still an open question. This limits the experiments we conducted and the corresponding results.
}
\end{itemize}




\subsection*{Review C}

\noindent {\bf Weaknesses}
The theoretical security analysis in this paper seems sound. Nevertheless, each parallel-chain protocol security analysis is not well-unified: the authors analyze the security of three adapted protocols (Prism, OHIE, and Fruitchains) independently. I agree that each parallel-chain protocol may have its own characteristics. However, as the authors have already proposed a generic methodology to add a variable mining difficulty on those parallel-chain protocols, it would be natural to use a unified framework (based on the methodology of M1, M2, and M3) to analyze the security of those protocols. Such a unified security proof framework would make this paper stronger. \re{Thanks for the suggestion. we reorganized the proof structure in a unified manner. The proofs are divided into three parts: (a) pivot chain properties, (b) non-pivot chain properties, (c) full protocol security. All three protocols need (a), Prism and OHIE need (b), and (c) depends on the specific ledger formation rule in each protocol.}

The experimental results in section 7 are insufficiently precise:
In Figure 11, how do the authors define the ``average forking rate'' of a parallel-chain protocol? \re{``Average forking rate of all parallel chains'' is defined as the ratio of the number of blocks not on the longest chain, to the number of blocks on the longest chain, across all the parallel chains. We made this clear in the revision.} And Figure 11 shows the experimental results of which protocol? \re{It shows a simulated mining process on 1001 parallel chains. Please see the updated Section \ref{sec:exp-setup} for more details.} The authors should mention it in the caption.
``our simulation focuses on measuring the difficulty adjustment and stability of each chain''. Where is the definition of ``stability'' of a chain? How to quantify it (do the authors refer to previous work for that term)? \re{Sorry for not defining the terms clearly. ``Stability'' means the forking rate. We have removed this notion and use forking rate consistently.} In Figures 11, 13, and 14, how long is the ``Time''? It is hard to read these figures without data on the x-axis. \re{In all evaluation figures, the time (x-axis) is from Jan 2, 2019 to Feb 20, 2020. We have updated the figures to include the starting and end dates.}

\noindent {\bf Minor concerns}
\begin{itemize}
    \item In section 6.3, I do not follow how the authors propose conditions 2-4. It's worth elaborating on how to achieve those conditions and if those conditions are the ``best'' lower bounds or upper bounds. \re{We justified those conditions. They are not the best bounds, but sufficient conditions for proof of security to go through. Tightening these parameters for efficiency is outside the scope of this paper.}
    \item Figures 1-10 are no vector graphics, the paper contains several typos. \re{We made sure the figures look good even after zooming in on the pdf by increasing the dpi. Thanks for catching the typos.}
    \item In figure 2, what does T2 mean? \re{T2 refers to the target used by the red block, we have labeled it in the figure.}
    \item I feel it is better to put Theorem 6.24 at the beginning of section 6.5, not at the end of section 6.4. \re{Thanks for the suggestion. We moved the theorem to the right place.}
\end{itemize}






==> simulations_todo.tex <==


3. Demonstrate variable difficulty adjustment using some simulations [LY]. 
    - show the difficulty adjustment works, with the number of players change
    --- X-axis = time, Y-axis has $Y_1$ (mining power) and $Y_2$ (difficulty). $Y_2$ tracks $Y_1$ with a lag as long as $Y_1$ is slowly varying. $Y_3$ is average inter-block time. $Y_4$ is the forking rate.
        ---- $Y_1(T)$ -> Bitcoin mining power variation (real-world) (take a rapid-changing section)
            ---- https://www.blockchain.com/charts/hash-rate
            
+++ Figures ready +++            

        ---- Long-range plot and a short range (2-epochs with focus on epoch boundary) plot. How does the difficulty on different chains vary? Short-term plots: 
            1. Push $f \delta$ to be high to show how the difficulty target oscillates. (Use $Unif[0,\Delta]$ as delay). We want to show the difficulty of each voter chain being non-monotonic for a short while
               OR, Craft a simulation where this effect happens at epoch boundary. 
            2. ANOTHER PLOT time vs. fraction of chains that have shifted to the new difficulty)
            3. ANOTHER PLOT How does ADV Behavior influence short term plots? CRAFTING adversarial behavior/scenario
                - intuitive: two proposer forks having very different difficulty
                - not so intuitive: adv refusing to adopt to new difficulty (show how long the adv can refuse to adopt the new 
                difficulty)
                - Two examples: Protocol where referred proposal chain difficulty has to be monotonic VS Protocol (straw-man) where this is not a validity requirement. Maybe show the forking rate if the adv can freely choose the anchor proposer block.
    --- Prism + Var Difficulty 
        ---- The scheme can maintain high throughput even with variable difficulty
            - Potential problem with the logic: if you wanted HT you should have ran Prism 1.0
            - Logic: Parallel chain can achieve high throughput and low latency. Now with this paper, you can get HT and low latency when there is variable difficulty. The outcome will not be surprising but will be good for adding strength to the paper.
            - One Possibility: Real Prism System
            
            
        [Skip latency]---- Latency: 
          - Prerequisite: replace counting levels with counting total difficulty, compare with 2md (d is proposer block difficulty)
            - can confirm a block, but we do not know the concrete confirmation probability
            - just to show that it is a well-defined proposal to apply the proposal to Prism fast confirmation

    - [skip] attacks
        ---- Demonstrate the difficulty raising attack (prob. of succeeding, etc.)
        ---- CAN monte carlo if there is no factor-4 bound. Maybe it is just focusing on the Bitcoin rule, instead of our contribution?
        
    
    - two consensus algorithms:
        - OHIE, Prism. We can plug the main idea into these two concrete protocols.
        - And they work
    
      


==> todo.tex <==

To DO
1. Complete the chain growth, chain prefix and 
chain quality. 
2. Liveness of Prism |->discuss the liveness proof.  [XW] [VV] - Friday Jan 8
3. Demonstrate variable difficulty adjustment using some simulations [LY]. 
    - show the difficulty adjustment works, with the number of players change
    - anything is good (even just replaying the formula)
    - two consensus algorithms:
        - OHIE, Prism. We can plug the main idea into these two concrete protocols.
        - And they work
    - attacks
        - Demonstrate the difficulty raising attack (prob. of succeeding, etc.)
    - Prism fast confirmation
        - Prerequisite: can we easily extend Xuechao's Prism confirmation rule to follow this paper? [XW]
            - can confirm a block, but we do not know the concrete confirmation probability
            - just to show that it is a well-defined proposal to apply the proposal to Prism fast confirmation
            - calculate the probability of private attack (difficulty raising) succeeding
                - Unsure: can we simulate this? What if the probability is very small?
            - calculate the latency
        
        
To write
1. State some variables and make some claims about the proposal chain, citing theorems from the other paper.  [VV]




Organization of the paper
1. Abstract [SK]
2. Introduction  [SK]
-Some explanation on the model here.
- How variable difficulty is handled in longest chain [Figure]
3. Prism - Algorithm
- Explain Prism algorithm [LY]
- Natural adaptations do not work [XW]
  -- Use different difficulty for diff chains
  -- Use same difficulty for diff chains but use levels.
     --- A1: Show an attack when voter chain can refer to proposal level non-monotonically
     --- A2: showing why referred proposal blocks should have monotonic difficulty (not monotonic levels)  (safety failure)
     --- choose a winner for each difficulty level rather than each depth level. (liveness failure)
Solution and  meta-principle [SK]

Meta-principle: 
- Use a single chain to decide difficulty for all chains
- Replace the notion of level with total-difficulty level everywhere in the algorithm. Note: Total-difficulty is a real number whereas level is a discrete index. Needs to be handled carefully.
- Use diff adjustment similar to Bitcoin.
- Full Prism algorithm with difficulty adjustment in English [XW,LY] [Figure]
Pseudocode [VV]
4. OHIE - Algorithm
-- Fixed diffuclty algorithm [Figures]
-- Variable difficulty algorithm [Figures]
5. Model [XW,VV]
  - Variable no of players. Assumptions on whether the function is fixed prior to execution or after. 
6. Proofs
   - Brainstorm figures  [XW,VV]
   -- Longest chain proof structure
   -- Parallel chain proof structure
   -- Logic flow explained in figures
   -- Proof adaptation to OHIE. 
7. Experiments [LY]

8. Discussion [SK]



--------
Figures
1. Prism standard figure
2. 


Viswa things to do [Jan 11]
1. Section 3.1 Prism basic algorithm 
 -  Prism standard figure 
 - Explain why it achieves fast confirmation  (look at Sec 4.1 of https://arxiv.org/pdf/1810.08092.pdf - end of page 7)
2. Section 3.2 Variable difficulty - Standard adpatations dont work
-----------


-----------
References:
1) 



Current sections
Abstract [SK]
1. Introduction [SK]
 - Related work 
2. Model [XW]
- Modeling whether adversary is allowed to see the execution in determining the future mining power. [To do: XW]
3. Prism [XW, VV]
4. OHIE [XW]
5. Security Analysis [XW,VV]
- Liveness figure [VV]
6. Simulations
7. Discussion [SK]

Appendix
A. Difficulty raising attack [XW]
B. Backbone properties revisited  [VV]

Terminology: 
Chain difficulty for chain and difficulty for block. 

-----------------
IMP Discussion on Fruitchains [XW]
 - Undecided whether to include this in paper. 
-----------------

viswa todo:
change chain prefix to common prefix [done]
chain quality - say that it follows the same argument from cp [done]
fixed difficulty sortition  [done]
expand appendix b [done?]
define stale chain [done]
liveness figure [done]
unify the notation [done?]
check if the references are correct and link to sections in the introduction
add 1-sentence summary in the abstract [done]
add $C^*$ in voter cp proof figure [done]
caption figures [done]
add references to martingale [done]
fix pseudo code

==> tokens.tex <==


Abstract  [SK] - Done
 - resolve open comments
 - using all three rules vs only some rules
Introduction  [SK] - Done
- resolve open comments
[VV] - Grammar and style [done]
[XW] - compare three related works on Bitcoin [done]
Model []

3. PRISM [SK] - Done
- call out sortition
- Fast confirmation what we need to write. 
4 - 6 [SK]

7. DONE [LY] Say specifically that simulations apply broadly
DONE [LY] Figure 14: typo in legend on delay. Inference => 
[LY] Figure 15: Long range plot with maybe 2 plots? one for ours one for M2
DONE [LY] Figure 12, add a curve for range of difficulty across chains.


[XW] Add a few lines about how incentives are done using short-term chain quality for Fixed Diff Fruitchains 
Add corresponding lines on variable difficulty. 
add a paragraph on main result. [done]

--------
Cross-paper tasks
1) VV: make sure all figures are referenced properly in text. [done]
make sure that M1, M2, M3 go into figures. 
DONE 2) LY: Edit figure captions
3) XW: References. Make sure to refer liberally. [emin-gun sirer paper on selfish-mining + variable difficulty]. Make sure there are no empty references [] or ? in the paper. 
4) XW: Integrate M1, M2, M3 into the paper. in the natural papers, [done]
5) VV: State main theorems in 3,4. [done]
